On the Inductive Bias of Stacking Towards Improving Reasoning

Given the increasing scale of model sizes, novel training strategies like gradual stacking [Gong et al., 2019, Reddi et al., 2023] have garnered interest. Stacking enables efficient training by gradually growing the depth of a model in stages and using layers from a smaller model in an earlier stage to initialize the next stage. Although efficient for training, the model biases induced by such growing approaches are largely unexplored. In this work, we examine this fundamental aspect of gradual stacking, going beyond its efficiency benefits. We propose a variant of gradual stacking called MIDAS that can speed up language model training by up to 40%. Furthermore we discover an intriguing phenomenon: MIDAS is not only training-efficient but surprisingly also has an inductive bias towards improving downstream tasks, especially tasks that require reasoning abilities like reading comprehension and math problems, despite having similar or slightly worse perplexity compared to baseline training. To further analyze this inductive bias, we construct reasoning primitives -- simple synthetic tasks that are building blocks for reasoning -- and find that a model pretrained with stacking is significantly better than standard pretraining on these primitives, with and without fine-tuning. This provides stronger and more robust evidence for this inductive bias towards reasoning. These findings of training efficiency and inductive bias towards reasoning are verified at 1B, 2B and 8B parameter language models. Finally, we conjecture the underlying reason for this inductive bias by exploring the connection of stacking to looped models and provide strong supporting empirical analysis.

==> Fig_Table/iso_plots_individual.tex <==
\begin{figure*}[H]% [H] is so declass\'e!
    \centering
    \begin{subfigure}{0.24\textwidth}
\centering    
    \includegraphics[width=\textwidth]{Media/iso_triviaqa.png}
    % \caption{}
    \label{fig:iso_triviaqa}
    \end{subfigure}\hfill
\centering
    \begin{subfigure}{0.24\textwidth}
    \centering    \includegraphics[width=\textwidth]{Media/iso_squadv2.png}
    % \caption{}
    \label{fig:iso_squadv2}
    \end{subfigure}\hfill
\centering
    \begin{subfigure}{0.24\textwidth}
    \centering    \includegraphics[width=\textwidth]{Media/iso_lambada.png}
    % \caption{}
    \label{fig:iso_lambada}
    \end{subfigure}\hfill
\centering
    \begin{subfigure}{0.24\textwidth}
    \centering    \includegraphics[width=\textwidth]{Media/iso_codedepth0.png}
    % \caption{}
    \label{fig:iso_codedepth0}
    \end{subfigure}\hfill
    \caption{\looseness-1Downstream eval vs log perplexity iso-plots as training proceeds for baseline and \method 1B models trained on the exact same data -- the stacking schedule used in this plot trains 24\% faster then baseline. Overall, as one would expect, downstream performance for both methods improves as log perplexity gets lower (towards the right side on the x-axis). For a memorization task like TriviaQA, baseline and \method have very similar downstream performance at the log perplexity. For tasks like SQuAD (open book QA) and Lambada (story completion), \method has better downstream performance at an equivalent log perplexity. This showcases the inductive bias of \method towards better quality.{}}
    \label{fig:iso_plots}
\end{figure*}



==> Fig_Table/primitives_summary.tex <==


\begin{figure*}[!th]% [H] is so declass\'e!
    \centering
    \includegraphics[width=0.8\textwidth]{Media/primitives_summary_bar_chart.png}
    \caption{\looseness-1Accuracy improvements for model trained with \method{} over baseline for representative \textit{reasoning primitives}, despite having the same perplexity.}
    \label
    \vspace*{-0.1in}
\end{figure*}
